Personalized Food Recommendation as Constrained Question Answering over a Large-scale Food Knowledge Graph

Food recommendation has become an important means to help guide users to adopt healthy dietary habits. Previous works on food recommendation either i) fail to consider users' explicit requirements, ii) ignore crucial health factors (e.g., allergies and nutrition needs), or iii) do not utilize the rich food knowledge for recommending healthy recipes. To address these limitations, we propose a novel problem formulation for food recommendation, modeling this task as constrained question answering over a large-scale food knowledge base/graph (KBQA). Besides the requirements from the user query, personalized requirements from the user's dietary preferences and health guidelines are handled in a unified way as additional constraints to the QA system. To validate this idea, we create a QA style dataset for personalized food recommendation based on a large-scale food knowledge graph and health guidelines. Furthermore, we propose a KBQA-based personalized food recommendation framework which is equipped with novel techniques for handling negations and numerical comparisons in the queries. Experimental results on the benchmark show that our approach significantly outperforms non-personalized counterparts (average 59.7% absolute improvement across various evaluation metrics), and is able to recommend more relevant and healthier recipes.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> other/04_Experiments_legacy.tex <==
\section{Experiments}

In this section, we evaluate our proposed PFoodRec model against competitive baseline methods on the personalized food recommendation benchmark.  
We also conduct extensive experiments to study the impact of each individual technique we introduce for handling personalization.
The dataset as well as the implementation of our model will be made publicly available after the review period.



\subsection{Baseline Methods}

Our main baseline is BAMnet~\cite{chen2019bidirectional}, a state-of-the-art neural network-based KBQA method
that directly retrieves answers from a KG subgraph by jointly embedding the question and KG subgraph.
% However, our \PBAMnet model extends BAMnet to treat food recommendation as a personalized KBQA problem by leveraging our
% proposed simple yet effective techniques including
% query expansion, KG augmentation and constraint modeling.
Besides, we also include a sophisticated embedding-based KBQA method called MatchNN which was motivated by \cite{bordes2014question}.
To demonstrate that this is a non-trival task, we further include a Bag-of-Word (BOW)~\cite{manning2008introduction} vectors based KBQA method as a baseline.
Whereas BAMnet encodes a question and each candidate answer jointly by considering the two-way flow of
interactions between them, in MatchNN and BOW baselines,
the question and candidate answers are encoded independently.
More specifically, for both MatchNN and BOW, the candidate answer is encoded as the sum of the corresponding answer type, answer path and answer context embeddings.
When embedding a question (or KG aspect such as answer type), MatchNN employs a bidirectional Long Short-Term Memory (LSTM)~\cite{hochreiter1997long} for encoding the sequence of tokens, 
and BOW simply takes the average of their pretrained word embeddings~\cite{pennington2014glove}.
Note that none of the above baselines explicitly handle personalized QA and they are included as non-personalized baselines in our experiments.


To examine whether our proposed techniques are generic enough and can be applied to extend regular KBQA methods for handling personalized food recommendation, we develop personalized versions of the aforementioned three KBQA baselines by leveraging our proposed simple yet effective techniques including query expansion, KG augmentation and constraint modeling.
Therefore, we have three personalized KBQA methods including P-BOW, P-MatchNN and \PBAMnet
where \PBAMnet is the main model proposed in this work.
Note that the personalized KBQA methods which leverage query expansion have access to the expanded query $\Tilde{q}$.








\subsection{Data and Metrics}

FoodKG~\cite{haussmann2019foodkg} is a large-scale knowledge graph that integrates recipes, food ontologies, and nutritional data.
It comprises approximately one million recipes (sourced from~\cite{marin2018learning}), 7.7 thousand nutrient records (sourced from the USDA: \url{www.usda.gov}), and 7.3 thousand classes of food (sourced from~\cite{griffiths2016foodon}). 
Overall, it has over 67 million triples. 
In this work, we use FoodKG as the underlying food knowledge graph.

ADA Lifestyle Management~\cite{american20195} includes ADA's current clinical practice recommendations and is intended to provide the components of diabetes care, general treatment goals and guidelines, and tools to evaluate quality of care. 
We carefully select food-related guidelines on nutrient and micronutrient needs for ``healthier'' food recommendation.

Following the steps described in~\cref{sec:benchmark_creation}, we create a QA style food recommendation benchmark based on FoodKG and ADA guidelines.






Following previous work on KBQA~\cite{berant2013semantic,chen2019bidirectional}, macro F1 scores (i.e., the average of F1 scores over all questions) are reported
on the test set.
F1 is a measure considering both the precision and the recall of the prediction to compute the score.
Besides F1, we also report Mean Average Precision (MAP) and Mean Average 
Recall (MAR) scores that are common metrics for evaluating recommender systems.
Basically, MAP gives insight into how relevant the recommended items are to the ground-truth responses, whereas MAR gives insight into how well a recommender system is able to recall items from the ground-truth answers.
Note that for all metrics, we consider all the answers returned by a system.








\subsection{Model Hyperparameter Settings}

%Below we describe the hyperparameter settings for the BAMnet and \PBAMnet models.
When constructing the vocabularies of words (from questions and KG), entity types (from KG) and relation
types (from KG), we only consider those questions and their corresponding KG subgraphs appearing in the training set.
The vocabulary sizes of words, entity types and relation types are 7009, 7 and 11, respectively.
% The vocabulary size of words is $V=7,009$. 
% There are 7 entity types and 11 relation types in the KG subgraphs.
% For those non-entity nodes which are boolean values or numbers, we use ``bool'' or ``num'' as their types, respectively. 
Given a topic entity, we extract its 2-hop subgraph
(i.e., $k=2$) to collect candidate answers, which is sufficient for our benchmark. 
% At training time, the memory size is limited to $N_{max} = 96$ candidate answers (for the sake of efficiency). 
% If there are more potential candidates, we do random sampling as mentioned earlier. 
We initialize word embeddings with 300-dimensional pre-trained GloVe vectors~\cite{pennington2014glove}.
% The relation embedding size $d_p$, entity type embedding size $d_t$  and hidden size $d$ are set as 128, 16 and 128, respectively.
% The dropout rates on the word embedding layer, question encoder side and the answer encoder side are 0.3, 0.3 and 0.2, respectively. 
The batch size is set as 32, and answer module threshold $\theta=1.8$. 
In the training process, we use the Adam optimizer
\cite{kingma2014adam}. We use $d_m=40$ for constraint modeling.
% (initial learning rate is 0.001, reduced by 10 if no improvement on validation set for 3 epochs; training stops if no improvement  on validation set for 10 epochs). 
All hyperparameters are tuned on the development set; for BAMnet we use the default values mentioned in Chen et al.~\shortcite{chen2019bidirectional}.




\subsection{Experimental Results}



\cref{table:exp_results} shows the evaluation results comparing our proposed method against other baseline methods.
\begin{table}[ht!]
\centering
\begin{tabular}{lllll}
\hline
 Method  & \vline & MAP & MAR & F1\\
  \hline
  \hline
 BOW &\vline& 1.8 & 1.8 & 2.0\\ 
 MatchNN &\vline & 2.5 & 2.4 & 2.6\\
 BAMnet &\vline& 2.5 & 2.4 & 2.7\\ 
 \hline
 P-BOW &\vline& 4.1 & 4.0 & 3.8\\
 P-MatchNN &\vline& 42.6 & 42.3 & 38.6\\
 \hline
 \PBAMnet &\vline& \bf{57.0} & \bf{56.2} & \bf{54.9}\\ 
\end{tabular}
% \vspace{-0.1in}
\caption{Experimental results (in \%) on the test set.}
\label{table:exp_results}
% \vspace{-0.1in}
\end{table}
We observe that the personalized systems significantly outperform their non-personalized counterparts, which demonstrates the effectiveness of our proposed techniques for 
utilizing the personal information (i.e., dietary preferences and health guidelines) to provide more accurate and personalized food recommendations
For example, the proposed \PBAMnet model consistently outperforms BAMnet by a significant margin (54.5\% absolute improvement in MAP, 53.8\% absolute improvement in MAR, and 52.2\% absolute improvement in F1 ) in all evaluation metrics.
Interestingly, the performance gap between BOW and P-BOW is not as significant as other KBQA methods.
This may be because the BOW technique for encoding the latent semantics is not very effective on this task.
Moreover, we can observe that there is still scope for improvement on this benchmark, which requires a certain level of reasoning to understand the different constraints in a query and to satisfy them based on the corresponding KG sub-graph. While \PBAMnet performs the best, the results indicate that our benchmark is quite challenging and can serve as a basis to spur further research in this fruitful area.




\subsection{Human Evaluation}

Properly evaluating and measuring the effectiveness of a good personalized food recommender means allowing for user subjectivity and differences in opinion on what factors are more important. For example, to a user, recipes violating only one constraint might be more preferable than recipes violating many, while to another, a recipe violating a nutritional guideline might be better than one violating an ingredient preference. A human evaluation allows for this user preference aspect of the recommendations to be evaluated.

We performed human evaluation for food recommendations by presenting a set of eight evaluators with fifty questions from a randomized test, along with the user personas spanning ingredient preferences (likes and dislikes) and applicable nutrition guidelines. For each question, we provide the answers from BAMnet, P-BOW, P-MatchNN and \PBAMnet models in a randomized order as shown in Figure \ref{fig:human_eval}. 
\begin{figure}[!t]
    \centering
    \centerline{
    \subfloat[Question Interface]{
    \includegraphics[
    scale=0.75
    ]{images/human_eval_v2.png}}}
    \centerline{
    \subfloat[Answer Set (0)]{
    \includegraphics[scale=0.4]{images/answer_set0.PNG}
    }}
    \caption{Snippet of Interface presented to human evaluators. (a) Each question is followed by Persona and Guideline entries. The shaded boxes link to the answer set comprising the top 3 answers from a given system. The ordering of the answer sets is randomized from one question to the next. (b) {\tt Answer 0} answer set for Question 0 in (a). Each response has the recipe title, followed by ingredients and nutrient information.}
    \label{fig:human_eval}
\end{figure}
Each answer presented to the user contains the top three recipes (if more than three recipes were retrieved), the ingredient list, and the nutritional values. The evaluators were instructed to rank the answers in the order of their (subjective) preference on a scale from $1-4$, with $1$ being the best, indicating which answer set they considered to be the best, without knowing which of the four systems generated the answers.
We adopt a simple rank aggregation strategy to compute the overall score for each system based on the ranks provided by human evaluators.
Specifically, we map the ranks 1, 2, 3 and 4 to the corresponding scores 10, 7, 4 and 1, so that systems with better ranks have higher scores.
Evaluation scores from all 8 evaluators are collected and averaged as final scores. 
As a result, the highest score a system can get is 10 while the lowest score is 1.
As shown in~\cref{table:human_evaluation_results}, our proposed \PBAMnet model achieves the best results compared to the other baselines. Furthermore, all of the personalized baselined fared better than the non-personized BAMnet approach. These resutls conclusive demonstrate the general applicability and effectiveness of our personalization techniques.



\begin{table}[!htb]
% \vspace{-4mm}
\begin{center}
% \addtolength{\tabcolsep}{-3.5pt}
\scalebox{1}{
\begin{tabular}{lll}
\hline
%   Methods & \vline & Syntactically correct & Semantically correct & Relevant \\
Method & \vline & Score \\
  \hline
BAMnet &\vline & 3.82 (0.70)\\
P-BOW &\vline & 4.69 (0.47)\\
P-MatchNN &\vline & 7.05 (0.44)\\
\hline
\PBAMnet &\vline & {\bf 7.76} (0.50)\\
\end{tabular}
}
\end{center}
\caption{Human evaluation results ($\pm$ standard deviation) on the test set. The rating scale is from 1 to 10 (higher scores indicate better results).}
\label{table:human_evaluation_results}
% \vspace{-3mm}
\end{table}









\subsection{Model Analysis}
% \subsection{Ablation Study}


\subsubsection{Ablation Study}

We perform an ablation study to systematically investigate the impact of different model components for our \PBAMnet method.
Here we briefly describe the ablated systems: 
\textrm{--} CM removes the Constraint Modeling module,
\textrm{--} KA removes the KG Augmentation module,
and \textrm{--} QE removes the Query Expansion module.
Note that for the ablated systems, we remove one module each time.

\begin{table}[ht!]
\centering
\begin{tabular}{lllll}
\hline
  Method & \vline & MAP & MAR  & F1\\
  \hline
  \hline
 \PBAMnet &\vline&57.0 & 56.2 & 54.9\\ 
 \qquad \textrm{--} KA &\vline& 54.4 & 53.8 & 52.7\\ 
 \qquad \textrm{--} CM &\vline& 28.4 & 27.9 & 20.2\\ 
 \qquad \textrm{--} QE &\vline& 3.8 & 3.7 & 3.6\\ 
\end{tabular}
% \vspace{-0.1in}
\caption{Ablation study (in \%) on the test set.}
\label{table:ablation_results}
% \vspace{-0.1in}
\end{table}

\cref{table:ablation_results} shows the experimental results of the above ablated systems as well as the full model.
It confirms our finding that all of the three techniques introduced for handling the personalized recommendation setting greatly contribute to the overall model performance.
Among them, the Query Expansion module contributes most, which demonstrates the  importance of incorporating rich personal information in order to provide accurate recommendation.
By removing the QE module, we observe an average 52.3\% performance drop across all evaluation metrics.
The CM module is also important as we see an average 30.5\% performance drop across all evaluation metrics if it is removed.
This shows the importance of handling negations for personalized food recommendation.
Lastly, the KA module also contributes to the overall model performance.

% Interestingly, \PBAMnet w/o CM only slightly outperforms the BAMnet baseline.
% We speculate this is because query expansion might not be that helpful for a model that cannot appropriately handle negations and
% thus might mistakenly retrieve candidates which satisfy negative constraints.
% Besides, the KA module also seems to be important.
% Similarly, without the capability of appropriately handling numerical comparison, we observed that \PBAMnet w/o KA cannot fully take advantage of the extra information brought by query expansion.
% Lastly, we find that even without query expansion, by applying our proposed CM techniques, \PBAMnet w/o QE actually outperforms BAMnet, which indicates that it is helpful to explicitly markup those constraints for a KBQA system.





\begin{table}[!htb]
\centering

\begin{tabular}{p{12cm}}
\hline
\multicolumn{1}{c}{\bf Test Query}\\
\hline
\textbf{Query:} Could you recommend eggplant dishes which do not contain ketchup?\\
\textbf{Preference:} Likes: [``white wine vinegar''], Dislikes: [``sesame'', ``red peppers'']\\
\textbf{Guideline:} Protein: 5.0 g to 30.0 g\\
\textbf{Gold:}  \textbf{[``Moussaka (Vegan or Vegetarian, You Choose.)'']}\\
\hline
~\\[-0.2in]
\multicolumn{1}{c}{\bf Baseline Methods}\\
\hline
\textbf{BOW:} [ ``Yunnan Style Grilled Veggies With Dipping Sauce'' ]  \\
\hline
\textbf{MatchNN:} [ ``Sicilian Eggplant Parmagiana With Spinach'', ``Savannah Dip'', ``The Real Melitzanosalata'', ``Eggplant, Tomato and Mozzarella Stacks, Hot or Cold'', ``The Ultimate Veggie Burger Thai Style'', ``Rigatoni With Roasted Eggplant Puree'', ... ] \\
\hline
\textbf{BAMnet:} [ ``Yunnan Style Grilled Veggies With Dipping Sauce'', ``Isabella\'s Gnocchi With Tomato and Eggplant Sauce'', ``The Real Melitzanosalata'', ``Savannah Dip'', ``The Ultimate Veggie Burger Thai Style'', ``Rigatoni With Roasted Eggplant Puree'', ... ]  \\
\hline
\textbf{P-BOW:} [ ``Black Cherry Tomatoes and Eggplant Pasta Sauce'', ``Italian Sausage and Eggplant Soup'', ``Clarica\'s Melitzanosalata'', ``Caponata'', ``Greek Eggplant Dip'', ... ]\\
%``Caponata (Caponatina)'', ... ] \\
\hline
\textbf{P-MatchNN:} [ ``White Bean Ratatouille'' ]\\
\hline
~\\[-0.2in]
\multicolumn{1}{c}{\bf Ablated Methods}\\
\hline
\textbf{\BlackPBAMnet w/o QE:} [ ``Yunnan Style Grilled Veggies With Dipping Sauce'', ``Isabella\'s Gnocchi With Tomato and Eggplant Sauce'', ``The Real Melitzanosalata'', ``Savannah Dip'', ``The Ultimate Veggie Burger Thai Style'', ``Rigatoni With Roasted Eggplant Puree'', ... ] \\
\textbf{\BlackPBAMnet w/o KA:} [ ``White Bean Ratatouille'' ]   \\
\textbf{\BlackPBAMnet w/o CM:}
[ ``Moussaka (Vegan or Vegetarian, You Choose.)'', ``White Summer Lasagna'', ``Pasta With Eggplant and Pork'', ``Leek and Chevre Lasagne'', ``Eggplant, Roasted Red Pepper and Brie Pasta'', ``Crazy Lasagna'', ... ]\\
\hline
~\\[-0.2in]
\multicolumn{1}{c}{\bf \BlackPBAMnet Method}\\
\hline
\BlackPBAMnet: [ ``Moussaka (Vegan or Vegetarian, You Choose.)'' ]\\
\hline
\end{tabular}

\caption{Predicted answers by various methods.}
\label{table:case_study}
\end{table}


\subsubsection{Case Study}


Table~\ref{table:case_study} shows the predicted 
answers from \PBAMnet and its ablated variants, and all of the baselines on an example from the test set.
In this example, the user is asking for eggplant dishes that do not contain ketchup. The user's persona includes both likes (e.g., white wine vinegar) and dislikes (e.g., red peppers), and a health/diet guideline for protein intake.
As we can see, \PBAMnet retrieves the ground-truth response from the KG while other systems make many imprecise recommendations.
For example,  
\PBAMnet w/o CM recommends dishes that contain ``red peppers'' such as ``Leek and Chevre Lasagne'' and ``Crazy Lasagna'' when the user dislikes ``red peppers''.
The same mistake is also made by other systems like \PBAMnet w/o QE, MatchNN, and BAMnet that recommend ``The Real Melitzanosalata''.
Without effectively utilizing the health guideline, many systems also recommend dishes that have protein values outside of the stipulated range.



%\subsubsection{Interpretability Analysis}





%Our method is able to offer good interpretability by visualizing the attention scores computed for input queries.
%As we can see from~\cref{fig:viz_attn}, 
%the attention network is able to focus more on important words that are actually part of the constraints when encoding input %queries.

%\begin{figure}[!htb]
%    \centering
%    \includegraphics[keepaspectratio=true,scale=0.25]{images/viz_pbamnet_1_3.png}
%    % \vspace{-0.1in}
%    \caption{Visualization of importance scores for query words.}
%    \label{fig:viz_attn}
    % \vspace{-0.2in}
%\end{figure}



